Step Sizes for Strong Stability Preservation with Downwind-biased Operators

Strong stability preserving (SSP) integrators for initial value ODEs preserve temporal monotonicity solution properties in arbitrary norms. All existing SSP methods, including implicit methods, either require small step sizes or achieve only first order accuracy. It is possible to achieve more relaxed step size restrictions in the discretization of hyperbolic PDEs through the use of both upwind- and downwind-biased semi-discretizations. We investigate bounds on the maximum SSP step size for methods that include negative coefficients and downwind-biased semi-discretizations. We prove that the downwind SSP coefficient for linear multistep methods of order greater than one is at most equal to two, while the downwind SSP coefficient for explicit Runge--Kutta methods is at most equal to the number of stages of the method. In contrast, the maximal downwind SSP coefficient for second order Runge--Kutta methods is shown to be unbounded. We present a class of such methods with arbitrarily large SSP coefficient and demonstrate that they achieve second order accuracy for large CFL number.

==> dwglm.lessold.tex <==
Reference \cite{spijker2007} includes Theorems on the SSP coefficient for
general linear methods and for downwind Runge-Kutta methods.  By combining
elements of the proofs of those results, one easily arrives at the following.

\begin{thm}
The SSP coefficient of the downwind general linear method \eqref{dwglm} 
is the largest $r\ge0$ such that the method can be written in the
form
\begin{align} \label{dwglm_sspform}
y_i^n & = \sum_{j=1}^{s+1} r_{ij} y_j^{n-1} 
         + \Dt \sum_{j=1}^{i-1} p_{ij} \left(y_j^n + \frac{\Dt}{r}F(y_j^n)\right)
         + \Dt \sum_{j=1}^{i-1} \tp_{ij} \left(y_j^n + \frac{\Dt}{r}\tF(y_j^n)\right)
\end{align}
with all coefficients $r_{ij},p_{ij},\tp_{ij}$ non-negative.
\end{thm}

Consider the application of \eqref{dwglm_sspform} to a linear problem:
\begin{align}
F(u) & = \mL u & \tF(u) & = \tL u,
\end{align}
and define $z=\Dt\mL,\tz=\Dt\tL$.  Then a straightforward induction
shows that the solution can be written as
\be \label{glm_dw}
u_n = \psi_1(z,\tz)u_{n-1}+\psi_2(z,\tz)u_{n-2}+\cdots+\psi_k(z,\tz)u_{n-k},
\ee
$k$ is the number of steps used in the method.

Since $\tlambda\approx-\lambda$, the method \eqref{glm_dw} approximates the 
solution of \eqref{testode} to order $p$ if
\be
\label{ocexp_dw}
e^{kz} = \psi_1(z,-z)e^{(k-1)z} + \psi_2(z,-z)e^{(k-2)z} + \cdots + \psi_k(z,-z) + \Oop(z^{p+1}),
\ee
Using \eqref{psi_a_dw} and equating coefficients in \eqref{ocexp_dw}
gives the order conditions:
\be \label{oc_a_dw}
\sum_{i=1}^k \sum_{j=0}^q \sum_{l=0}^j (-1)^l a_{ijl} \frac{(k-i)^{p-j}}{(p-j)!}
= \frac{k^p}{p!} \quad \quad 1\le q \le p.
\ee


In this section we investigate the SSP coefficient for general linear 
methods with downwinding, when applied to the linear, constant coefficient
IVP
\begin{align} \label{linODE} u'(t) & =\mL u \end{align}
resulting perhaps from an upwind-biased semi-discretization of a linear 
hyperbolic PDE.  We consider additionally the system
\begin{align} \label{dwlinODE} u'(t) & =-\tL u \end{align}
obtained from the corresponding downwind-biased semi-discretization.
Typically $\tL=-\mL\transpose$.
We assume that these semi-discretizations satisfy the forward Euler
conditions
\begin{align}
\|\mI+\Dt\mL\| & \le 1 \mbox{ for } 0\le \Dt\le \DtFE \\
\|\mI+\Dt\tL\| & \le 1 \mbox{ for } 0\le \Dt\le \DtFE.
\end{align}

Applying a downwind Runge-Kutta method to this linear, 
constant-coefficient problem yields a recursion 
$$u^n = \psi(z,\tz)u^{n-1}$$ 
%The function $\psi(z,\tz)$
%will be referred to as the stability function of the method.
We will consider the larger class of downwind general linear methods, 
which use multiple stages and multiple previous steps to compute $u^n$, 
and for this linear problem lead to the recursion
\be \label{glm_dw}
u_n = \psi_1(z,\tz)u_{n-1}+\psi_2(z,\tz)u_{n-2}+\cdots+\psi_k(z,\tz)u_{n-k},
\ee
Where $s$ is the number of stages and $k$ is the number of steps
used in the method.
For explicit methods, the functions $\psi_i$ are polynomials with 
combined degree $s$:
\begin{align} \label{psi_a_dw}
\psi_i & = \sum_{j=0}^s \sum_{l=0}^j a_{ijl}z^{j-l}\tz^l & 1 \le i \le k.
\end{align}

The maximal strong stability preserving timestep 
for these methods is related to the radius of absolute monotonicity of
the functions $\psi(z,\tz)$, which we recall from \cite{higueras2006}.

\begin{dfn}
The radius of absolute monotonicity $\tR(\psi)$ of $\psi: \Re\to\Re^2$ is the 
largest value $r\ge0$ such
that all partial derivatives of $\psi(z,\tz)$ are non-negative for 
$z,\tz\in(-r,0]$.
\end{dfn}

In order to study the absolute monotonicity of a bivariate polynomial
$\psi(z,\tz)$, it is helpful to write it in the following form:
\be \label{dwtaylor}
\psi_i(z,\tz)= \sum_{j=0}^s \sum_{l=0}^j \gamma_{ijl}(r) 
  \left(1+\frac{z}{r}\right)^{j-l} \left(1+\frac{\tz}{r}\right)^{l}
  \quad \quad \mbox{with } \gamma_{ijl}(r) = \frac{r^j}{j!}\dd{^j\psi_i}{z^{j-l} \partial \tz^{l}}
\ee

\begin{lem} \label{leftend2}
A bivariate polynomial $\psi(z,\tz)$ is absolutely monotonic at $-\xi<0$ if 
and only if $\psi$ has radius of absolute monotonicity $R(\psi)\ge \xi$.
\begin{proof}
Suppose $R(\psi)\ge \xi$; then $\psi$ is absolutely monotonic at $-\xi$
by continuity.  On the other hand, suppose $\psi$ is absolutely monotonic 
at $-\xi$.  Write $\psi$ in the form \eqref{dwtaylor}.  Then 
term-by-term differentiation shows that $\psi$ is absolutely monotonic
on $(-\xi,0]$.
\end{proof}
\end{lem}
Thus we have
\be r \le \tR(\psi_i) \iff \gamma_{ijl}(r)\ge 0 \quad \mbox{for all } 0\le j\le i \le s
\ee

\begin{thm} \label{dwthm}
{\bf Can we/should we make this an iff statement?}

Let $||\cdot||$ be any convex functional and suppose $\mL,\tL$ satisfy the 
circle conditions \eqref{FEcond} and \eqref{dwFEcond}.
Then the monotonicity condition \eqref{monotonicity} holds for the solution of 
the linear autonomous pair \eqref{linODE}-\eqref{dwlinODE} by method 
\eqref{glm_dw} if the timestep satisfies
\be
\label{timestep2}
\Dt \le \tilde{R} \Dt_{FE}
\ee
where the threshold factor $\tilde{R}=\min_i R(\psi_i(z,\tilde{z}))$.
\end{thm}
\begin{proof}
Using \eqref{dwtaylor},
\begin{eqnarray*}
||\bu^{n}|| & = & ||\sum_i \psi_i(\Dt \mL,\Dt\tL)\bu_{n-i}|| \\
 & \le & \left\|\sum_i \sum_{j=0}^s \sum_{l=0}^j \gamma_{ijl}(r)
  \left(1+\frac{\Dt}{r}\mL\right)^{j-l} \left(1+\frac{\Dt}{r}\tL\right)^{l}\right\| \\
 & \le & \sum_{i,j,l} \gamma_{ijl}(r) \left|\left|\left(I+\frac{\Dt}{r}\mL \right)\right|\right|^{j-l} \left|\left|\left(I+\frac{\Dt}{r}\tL \right)\right|\right|^l  ||\bu_{n-i}||\\
 & \le & \sum_{i,j,l} \gamma_{ijl}(r) ||\bu_{n-i}|| \le \max_l ||\bu_{n-i}||.
\end{eqnarray*}
Here we have used the fact that $\sum_{i,j,l} \gamma_{ijl}(r) = 1$, which
holds for any consistent method.
\end{proof}

For a more general consideration of absolutely monotonic functions
that arise from considering downwind-biased methods, see 
\cite{higueras2005a,higueras2006}.

Let $\tilde{\Pi}_{s,k,p}$ denote the 
set of all ordered sets of $k$ bivariate polynomials 
$\{\psi_1,...,\psi_k\}$ of degree 
at most $s$ satisfying the order conditions \eqref{oc_a_dw} up to order $p$.

\begin{dfn} \label{dw-tf}
For given integers $s,k,p$, the {\em optimal downwind threshold factor}
$\tR_{s,k,p}$
is the largest threshold factor among all $k$-step, $s$-stage, order $p$
accurate general linear methods with downwinding:
\be
\tR_{s,k,p} = \sup\left\{\min_i \tR(\psi_i) \ | \ \{\psi_1,...,\psi_k\}\in \tilde{\Pi}_{s,k,p}\right\}.
\ee
\end{dfn}

Below, we will determine values of $\tR_{s,k,p}$
and corresponding optimal methods.  By virtue of Theorem \ref{dwthm} 
these methods are optimal in terms of the maximum timestep for contractivity.

The following corollary follows from Lemma \ref{leftend2} and Definition
\ref{dw-tf}.

\begin{cor} \label{bisectlem2}
Let $r>0$.  Then $\tR_{s,k,p}\ge r$ if and only if there exists 
$\{\psi_1,...,\psi_k\}\in \tilde{\Pi}_{s,k,p}$ such that each $\psi_i(z,\tz)$ 
is absolutely monotonic at $-r$.
\end{cor}

The next theorem provides an upper bound on $\tR_{s,k,p}$.  
Its proof, is very similar to that of \cite[Theorem~?]{gottlieb2009}
\begin{thm} \label{dwrmaxthm}
For any $s,k,p>0$, the optimal downwind threshold factor for 
explicit $s$-stage, $k$-step, order $p$ general linear methods 
is at most equal to the number of stages; i.e., $\tR_{s,k,p}\le s$.
\end{thm}
\begin{proof}
Take any $(\psi_1,...,\psi_k)\in \Pi_{s,k,p}$, and let $R$ be the threshold 
factor of this method.
Writing out explicitly the first two order conditions (i.e., \eqref{ocglm}
for $p=0,1$, with $r=R$) gives
\begin{subequations}
\label{oc01b}
\begin{align}
\label{oc01bi}
& \sum_{i=1}^k \sum_{j=0}^s \sum_{l=0}^j \gamma_{ijl} = 1,     \\
& \sum_{i=1}^k \sum_{j=0}^s \sum_{l=0}^j \gamma_{ijl} \left(j-2l + R(k-i)\right) = kR.
\label{oc01bii}
\end{align}
\end{subequations}
Since the $\gamma$'s are positive and sum to unity, then using the 
last equation above we have
\begin{align*}
kR & = \sum_{i=1}^k \sum_{j=0}^s \sum_{l=0}^j \gamma_{ijl} \left(j-2l + R(k-i)\right) \\
   & \le \max_{i\in(1,k),j\in(0,s),l\in(0,j)} \left(j-2l + R(k-i)\right) \\
   & = s + R(k-1).
\end{align*}
Subtracting $R(k-1)$ from both sides of this inequality gives
\be
R\le s.
\ee
\end{proof}




==> dwglm.old.tex <==
%In order to study linear accuracy and stability properties of downwind methods,
%we consider the usual test problem
%\be \label{testode} u'(t) = \lambda u,  \ee
%along with an additional "downwind discretization" of this problem:
%\be u'(t) = -\tlambda u,  \ee
%where $-\tlambda\approx\lambda$.

Since $\tlambda\approx-\lambda$, the method \eqref{glm_dw} approximates the 
solution of \eqref{testode} to order $p$ if
\be
\label{ocexp_dw}
e^{kz} = \psi_1(z,-z)e^{(k-1)z} + \psi_2(z,-z)e^{(k-2)z} + \cdots + \psi_k(z,-z) + \Oop(z^{p+1}),
\ee
Using \eqref{psi_a_dw} and equating coefficients in \eqref{ocexp_dw}
gives the order conditions:
\be \label{oc_a_dw}
\sum_{i=1}^k \sum_{j=0}^q \sum_{l=0}^j (-1)^l a_{ijl} \frac{(k-i)^{p-j}}{(p-j)!}
= \frac{k^p}{p!} \quad \quad 1\le q \le p.
\ee


In this section we investigate the SSP coefficient for general linear 
methods with downwinding, when applied to the linear, constant coefficient
IVP
\begin{align} \label{linODE} u'(t) & =\mL u \end{align}
resulting perhaps from an upwind-biased semi-discretization of a linear 
hyperbolic PDE.  We consider additionally the system
\begin{align} \label{dwlinODE} u'(t) & =-\tL u \end{align}
obtained from the corresponding downwind-biased semi-discretization.
Typically $\tL=-\mL\transpose$.
We assume that these semi-discretizations satisfy the forward Euler
conditions
\begin{align}
\|\mI+\Dt\mL\| & \le 1 \mbox{ for } 0\le \Dt\le \DtFE \\
\|\mI+\Dt\tL\| & \le 1 \mbox{ for } 0\le \Dt\le \DtFE.
\end{align}

Applying a downwind Runge-Kutta method to this linear, 
constant-coefficient problem yields a recursion 
$$u^n = \psi(z,\tz)u^{n-1}$$ 
where $z=\Dt\mL,\tz=\Dt\tL$.  
%The function $\psi(z,\tz)$
%will be referred to as the stability function of the method.
We will consider the larger class of downwind general linear methods, 
which use multiple stages and multiple previous steps to compute $u^n$, 
and for this linear problem lead to the recursion
\be \label{glm_dw}
u_n = \psi_1(z,\tz)u_{n-1}+\psi_2(z,\tz)u_{n-2}+\cdots+\psi_k(z,\tz)u_{n-k},
\ee
Where $s$ is the number of stages and $k$ is the number of steps
used in the method.
For explicit methods, the functions $\psi_i$ are polynomials with 
combined degree $s$:
\begin{align} \label{psi_a_dw}
\psi_i & = \sum_{j=0}^s \sum_{l=0}^j a_{ijl}z^{j-l}\tz^l & 1 \le i \le k.
\end{align}

The maximal strong stability preserving timestep 
for these methods is related to the radius of absolute monotonicity of
the functions $\psi(z,\tz)$, which we recall from \cite{higueras2006}.

\begin{dfn}
The radius of absolute monotonicity $\tR(\psi)$ of $\psi: \Re\to\Re^2$ is the 
largest value $r\ge0$ such
that all partial derivatives of $\psi(z,\tz)$ are non-negative for 
$z,\tz\in(-r,0]$.
\end{dfn}

In order to study the absolute monotonicity of a bivariate polynomial
$\psi(z,\tz)$, it is helpful to write it in the following form:
\be \label{dwtaylor}
\psi_i(z,\tz)= \sum_{j=0}^s \sum_{l=0}^j \gamma_{ijl}(r) 
  \left(1+\frac{z}{r}\right)^{j-l} \left(1+\frac{\tz}{r}\right)^{l}
  \quad \quad \mbox{with } \gamma_{ijl}(r) = \frac{r^j}{j!}\dd{^j\psi_i}{z^{j-l} \partial \tz^{l}}
\ee

\begin{lem} \label{leftend2}
A bivariate polynomial $\psi(z,\tz)$ is absolutely monotonic at $-\xi<0$ if 
and only if $\psi$ has radius of absolute monotonicity $R(\psi)\ge \xi$.
\begin{proof}
Suppose $R(\psi)\ge \xi$; then $\psi$ is absolutely monotonic at $-\xi$
by continuity.  On the other hand, suppose $\psi$ is absolutely monotonic 
at $-\xi$.  Write $\psi$ in the form \eqref{dwtaylor}.  Then 
term-by-term differentiation shows that $\psi$ is absolutely monotonic
on $(-\xi,0]$.
\end{proof}
\end{lem}
Thus we have
\be r \le \tR(\psi_i) \iff \gamma_{ijl}(r)\ge 0 \quad \mbox{for all } 0\le j\le i \le s
\ee

\begin{thm} \label{dwthm}
{\bf Can we/should we make this an iff statement?}

Let $||\cdot||$ be any convex functional and suppose $\mL,\tL$ satisfy the 
circle conditions \eqref{FEcond} and \eqref{dwFEcond}.
Then the monotonicity condition \eqref{monotonicity} holds for the solution of 
the linear autonomous pair \eqref{linODE}-\eqref{dwlinODE} by method 
\eqref{glm_dw} if the timestep satisfies
\be
\label{timestep2}
\Dt \le \tilde{R} \Dt_{FE}
\ee
where the threshold factor $\tilde{R}=\min_i R(\psi_i(z,\tilde{z}))$.
\end{thm}
\begin{proof}
Using \eqref{dwtaylor},
\begin{eqnarray*}
||\bu^{n}|| & = & ||\sum_i \psi_i(\Dt \mL,\Dt\tL)\bu_{n-i}|| \\
 & \le & \left\|\sum_i \sum_{j=0}^s \sum_{l=0}^j \gamma_{ijl}(r)
  \left(1+\frac{\Dt}{r}\mL\right)^{j-l} \left(1+\frac{\Dt}{r}\tL\right)^{l}\right\| \\
 & \le & \sum_{i,j,l} \gamma_{ijl}(r) \left|\left|\left(I+\frac{\Dt}{r}\mL \right)\right|\right|^{j-l} \left|\left|\left(I+\frac{\Dt}{r}\tL \right)\right|\right|^l  ||\bu_{n-i}||\\
 & \le & \sum_{i,j,l} \gamma_{ijl}(r) ||\bu_{n-i}|| \le \max_l ||\bu_{n-i}||.
\end{eqnarray*}
Here we have used the fact that $\sum_{i,j,l} \gamma_{ijl}(r) = 1$, which
holds for any consistent method.
\end{proof}

For a more general consideration of absolutely monotonic functions
that arise from considering downwind-biased methods, see 
\cite{higueras2005a,higueras2006}.

Let $\tilde{\Pi}_{s,k,p}$ denote the 
set of all ordered sets of $k$ bivariate polynomials 
$\{\psi_1,...,\psi_k\}$ of degree 
at most $s$ satisfying the order conditions \eqref{oc_a_dw} up to order $p$.

\begin{dfn} \label{dw-tf}
For given integers $s,k,p$, the {\em optimal downwind threshold factor}
$\tR_{s,k,p}$
is the largest threshold factor among all $k$-step, $s$-stage, order $p$
accurate general linear methods with downwinding:
\be
\tR_{s,k,p} = \sup\left\{\min_i \tR(\psi_i) \ | \ \{\psi_1,...,\psi_k\}\in \tilde{\Pi}_{s,k,p}\right\}.
\ee
\end{dfn}

Below, we will determine values of $\tR_{s,k,p}$
and corresponding optimal methods.  By virtue of Theorem \ref{dwthm} 
these methods are optimal in terms of the maximum timestep for contractivity.

The following corollary follows from Lemma \ref{leftend2} and Definition
\ref{dw-tf}.

\begin{cor} \label{bisectlem2}
Let $r>0$.  Then $\tR_{s,k,p}\ge r$ if and only if there exists 
$\{\psi_1,...,\psi_k\}\in \tilde{\Pi}_{s,k,p}$ such that each $\psi_i(z,\tz)$ 
is absolutely monotonic at $-r$.
\end{cor}

The next theorem provides an upper bound on $\tR_{s,k,p}$.  
Its proof, is very similar to that of \cite[Theorem~?]{gottlieb2009}
\begin{thm} \label{dwrmaxthm}
For any $s,k,p>0$, the optimal downwind threshold factor for 
explicit $s$-stage, $k$-step, order $p$ general linear methods 
is at most equal to the number of stages; i.e., $\tR_{s,k,p}\le s$.
\end{thm}
\begin{proof}
Take any $(\psi_1,...,\psi_k)\in \Pi_{s,k,p}$, and let $R$ be the threshold 
factor of this method.
Writing out explicitly the first two order conditions (i.e., \eqref{ocglm}
for $p=0,1$, with $r=R$) gives
\begin{subequations}
\label{oc01b}
\begin{align}
\label{oc01bi}
& \sum_{i=1}^k \sum_{j=0}^s \sum_{l=0}^j \gamma_{ijl} = 1,     \\
& \sum_{i=1}^k \sum_{j=0}^s \sum_{l=0}^j \gamma_{ijl} \left(j-2l + R(k-i)\right) = kR.
\label{oc01bii}
\end{align}
\end{subequations}
Since the $\gamma$'s are positive and sum to unity, then using the 
last equation above we have
\begin{align*}
kR & = \sum_{i=1}^k \sum_{j=0}^s \sum_{l=0}^j \gamma_{ijl} \left(j-2l + R(k-i)\right) \\
   & \le \max_{i\in(1,k),j\in(0,s),l\in(0,j)} \left(j-2l + R(k-i)\right) \\
   & = s + R(k-1).
\end{align*}
Subtracting $R(k-1)$ from both sides of this inequality gives
\be
R\le s.
\ee
\end{proof}



